Dynamical fitness models: evidence of universality classes for preferential attachment graphs

In this paper we define a family of preferential attachment models for random graphs with fitness in the following way: independently for each node, at each time step a random fitness is drawn according to the position of a moving average process with positive increments. We will define two regimes in which our graph reproduces some features of two well known preferential attachment models: the Bianconi-Barab\'asi and the Barab\'asi-Albert models. We will discuss a few conjectures on these models, including the convergence of the degree sequence and the appearance of Bose-Einstein condensation in the network when the drift of the fitness process has order comparable to the graph size.

==> packages.tex <==


\usepackage{mathrsfs}
\usepackage{bbm,amssymb,mathtools}
\usepackage{comment}
\usepackage{xcolor}
\usepackage{nicefrac,bm}
\usepackage[titletoc]{appendix}
\usepackage{enumitem}
\makeatletter
\def\namedlabel#1#2{\begingroup
    #2%
    \def\@currentlabel{#2}%
    \phantomsection\label{#1}\endgroup
}
\makeatother
\usepackage{tikz}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother



\usepackage[a4paper,vmargin={3.5cm,3.5cm},hmargin={2.5cm,2.5cm},bottom=30mm]{geometry} %This sets better margins
\pdfoutput=1
\PassOptionsToPackage{hyphens}{url}
\usepackage{hyperref}% This is for hyperlinks
\hypersetup{colorlinks=true, linkcolor=blue, citecolor=blue,  filecolor=blue, urlcolor=blue}

  %%%Load url and hyperref before biblatex
\usepackage[backend=bibtex,style=authoryear,firstinits=true,isbn=false,doi=false,url=false,citestyle=authoryear-comp]{biblatex}
\renewcommand*{\multicitedelim}{\addcomma\space}
\addbibresource{refs.bib} %For bibliography
% New package option since 2019/10/02 update: font
\usepackage[sc,osf]{mathpazo}
\usepackage{graphicx}
\usepackage[utf8]{inputenc}

\usepackage{ifdraft}
\usepackage[draft]{changes}
\definechangesauthor[name={ale}, color=orange]{ale}
%New 'Remark' command
\makeatletter
\newcommand{\Changes@Markup@Remark}[1]{\textbf{NOTE:} #1}
\newcommand{\remark}[2][\@empty]{%
    \ifoptionfinal{}{
        \setkeys{Changes@added}{#1}%
        \Changes@output%
            {\Changes@Markup@Remark{#2}}%
            {#2}%
            {\Changes@added@id}%
            {\Changes@added@remark}%
            {#2}%
            {\changesaddname}%
            {\Changes@added@dec}%
            {\Changes@added@decid}%
            {\Changes@added@decremark}%
        \stepcounter{Changes@AddCount\Changes@added@id}%
    }
}
\makeatother



\newcommand{\bo}[1]{\mathbf{#1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\p}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\im}{\mathrm{i}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\eps}{\epsilon}

\newcommand{\F}{\mathscr{F}}
\newcommand{\D}{\mathscr{D}}
\newcommand{\T}{\mathscr{T}}
\newcommand{\PP}{\mathscr{P}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\Ep}{\mathcal{E}}
\newcommand{\Fit}{\mathcal{F}}
\newcommand{\ip}{\left\langle\,,\right\rangle}
\newcommand{\supp}{\mathrm{supp}}
\renewcommand{\div}{\mathrm{div}}
\newcommand{\cphi}{\phi}
\renewcommand{\phi}{\varphi}
\newcommand{\tphi}{\widetilde{\varphi}}
\renewcommand{\bar}{\overline}
\newcommand{\de}{\mathrm{d}}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}



\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\sk}{\vspace*{\baselineskip}}
\newcommand{\scs}{\scriptsize}
\newcommand{\I}{I_f^\epsilon}
\newcommand{\cv}{(\ref{convres}) }
\setlength\parindent{0pt}
\newcommand{\Ric}{\text{Ric}}


  
  \numberwithin{equation}{section} %This is for enumerating equations
 

%\newcommand{\grad}{\mathrm{grad}}
\newcommand{\grad}{\nabla}

%This is to define better the environment Paragraph
\makeatletter
\def\paragraph{\@startsection{paragraph}{4}%
  \z@\z@{-\fontdimen2\font}%
  {\normalfont\itshape}}
  \makeatother

  
  %% Def subsubsection
  
 \makeatletter
\def\subsubsection{\@startsection{subsubsection}{3}%
  \z@\z@{-\fontdimen2\font}%
  {\normalfont\scshape}}
  \makeatother
  %%%%%%%%
  
\theoremstyle{definition}
%\theoremstyle{mystyle}
\newtheorem{defi}{Definition}[section]
\newtheorem{rmk}[defi]{Remark}
\newtheorem{lemma}[defi]{Lemma}
\newtheorem{ex}[defi]{Example}
\newtheorem{claim}[defi]{Claim}

\theoremstyle{plain}
%\theoremstyle{mystyle2}
\newtheorem{thm}[defi]{Theorem}
\newtheorem{prop}[defi]{Proposition}
\newtheorem{cor}[defi]{Corollary}
\newtheorem{conj}[defi]{Conjecture}




